Conjugate Gradients for Kernel Machines

Regularized least-squares (kernel-ridge / Gaussian process) regression is a fundamental algorithm of statistics and machine learning. Because generic algorithms for the exact solution have cubic complexity in the number of datapoints, large datasets require to resort to approximations. In this work, the computation of the least-squares prediction is itself treated as a probabilistic inference problem. We propose a structured Gaussian regression model on the kernel function that uses projections of the kernel matrix to obtain a low-rank approximation of the kernel and the matrix. A central result is an enhanced way to use the method of conjugate gradients for the specific setting of least-squares regression as encountered in machine learning. Our method improves the approximation of the kernel ridge regressor / Gaussian process posterior mean over vanilla conjugate gradients and, allows computation of the posterior variance and the log marginal likelihood (evidence) without further overhead.

==> tex/discussion.tex <==
%\subsection{Open questions}
\label{sec:discussion}
%\todo{
%During exploratory experiments we found that the residual norm can not decrease sufficiently until almost the last step.
%}
%Our algorithm is theoretically faster than exact inference but in practice Cholesky decomposition is implemented just more efficiently.
%Still our algorithm is useful in settings where such an implementation is not available, e.g. in embedded systems.
%There are several possible directions to make our approach competitive.
%An advantage of \kmcg{} (compared to \pname{DTC}) is the possibility to carry over computational investments during hyper-parameter optimization.
Preconditioning as suggested by \citet{davies2015effectiveGPimplementation} or Krylov-subspace recycling \citep{Saad1999deflated} are promising ideas to improve \kmcg{} further.
%For example we found in exploratory experiments that preconditioning can actually worsen the condition of the linear equation systems.
%Another encouraging direction is Krylov-subspace recycling \citep{Saad1999deflated} where one computes approximate Eigenvectors $\vec U$ for $\vec K$ from $\vec S$ and uses these $\vec U$ as first search directions for the next problem.
%We found that this approach can reduce the number of necessary conjugate gradient iterations and it has furthermore the advantage that the multiplication with $\vec U$ can be executed as matrix-matrix product.
%However, as of now it is unclear to us how to decide how many approximate Eigenvectors to compute and which to actually use (for actual speed-up it is crucial not to take all). 

%Another issue not mentioned so far occurs also during hyper-parameter optimization.
%Calculating gradients with respect to the likelihood requires rerunning conjugate gradients with the same number of steps on $\partial \vec K$.
%We experimented with approximate gradients treating $\vec S$ independent of the kernels parameters.
%It appears that this approximation worsens the more conjugate gradient steps were taken.
%A bad approximation can cause the optimizer's line-search to fail if a descent direction did not decrease the likelihood.
%Likelihood optimization is an issue we will have to leave for future work.

%Our CG algorithm can speed up hyper-parameter optimization in the initial phase, when the matrix is badly conditioned and the kernel parameters do not fit the data.
%The results presented in Section \ref{sec:} are rather depressing.

%We explore these ideas in the next section.

%It remains an open question why conjugate gradients produces such unreliable estimates.
%The systematic replacement of $k$ appears to provide a reasonable explanation why our approach works.
%Nevertheless, (when the inducing inputs are a subset of the data) the predictive-mean (Equation \ref{eq:mean_scg}) can be written as $\vec k_*\Trans \vec \alpha$ for an $\vec \alpha \in \Re^N$.
%Therefore it is a-priori not clear why conjugate gradients does not produce a similarly well performing sequence of estimates $\vec \alpha$.


%The approximation works if there is more data than the class has capacity.

%Probably \pname{Variational Free Energy} does not arise from this framework. 
%Therefore our framework probably needs some work for better hyper-parameter tuning. 
%Nevertheless, finally one can use conjugate gradients.

%A question we left unanswered is how to choose the number of steps $P$ and the number of inducing points $M$. 
%However, this is typically a problem.
%To the best of our knowledge it is not even clear how many inducing points to choose for a good approximation.
%Empirically ... seems to work fine.

%\section{Open questions}
%Open question is how to make this an online algorithm.
%Approach needs the whole dataset in one attempt.
%Batch learning becomes necessary to compete with deep learning.
%\todo{cite batch variational-inference paper}

%\todo{using a $\ksig$ that is not $k$}

%\subsection{Future work}



==> tex/evaluation.tex <==
\label{sec:experiments}
%In this section we describe two kinds of experiments.
In this section we want to shed light on three questions. %from an empirical perspective.
First, we want to know how our approach of using conjugate gradients compares against the standard procedure.
Furthermore we explore the usefulness of our method as means to speed up GP hyper-parameter optimization for moderately sized datasets ($N\approx 5000$).
The \pname{automated statistician} \citep{Duvenaud2013structure} is an example of a practical scenario where this speed-up would be useful.
Third, we evaluate the scaling of our uncertainty measure in comparison to the approximation error.

We run the classical conjugate gradients algorithm to solve the equations $(\vec K +\noise\vec I)\vec x = \vec y$.
In contrast, since the goal of our algorithm is to learn an approximation to the kernel, our algorithm runs conjugate gradients on $\vec K \vec x = \vec y$, i.e.~without noise term.
Both algorithms are stopped when the relative residual ($\nicefrac{||\vec b - \vec A \vec x||_2}{||\vec b||_2}$) is smaller than $0.01$ or as soon as execution exceeds the time necessary for Cholesky decomposition.
We employ a slightly different implementation of conjugate gradients, constructing $\hat{\vec x}$ and the search directions $\vec S$ in a more stable way.
The details are described in Appendix \ref{app:implementation}.
Our implementation is based upon the evaluation framework proposed by \cite{chalupka2013comparison} where we conjugate gradients is a mex-routine employing Eigen.

For different datasets (see Table \ref{tbl:datasets}) from the UCI machine learning repository (\url{archive.ics.uci.edu/ml}) we evaluate the quality of approximation in terms of average relative error on the test set
%standardized mean squared-error (SMSE) \citep[p. 23]{Rasmussen.2006}, 
%\begin{align}
%\operatorname{SMSE}=\frac{1}{n_*}\sum_{k=1}^{n_*}\frac{\left(y_{*k}-\mu_{*k}\right)^2}{\operatorname{Var}[\vec y_*]},
%\end{align}
\begin{align}
\frac{1}{n_*}\sum_{k=1}^{n_*}\left|\frac{\y_{*k}-\mu_{*k}}{y_{*k}}\right|,
\end{align}
where $\vec y_*$ is the mean prediction of the exact Gaussian process in the test locations and $\vec \mu_*$ is the approximate mean prediction.
In all our experiments we used two popular kernel functions, namely automatic relevance determination (ARD) Squared Exponential (Eq.~\ref{eq:sq_exp}) and ARD Mat\'ern $\nicefrac{5}{2}$ \citep[p. 83f, p. 106]{RasmussenWilliams}, 
\begin{align}
\label{eq:matern}
k_{52}(d(\vec x,\vec z; \vec \Lambda))&=f\left(1+\sqrt{5}d+\frac{5}{3}d^2\right)\exp{\left(-\sqrt{5}d\right)}
\end{align}
where $d=d(\vec x, \vec z; \vec \Lambda)=||\vec x-\vec z||_{{\vec \Lambda}}$ and $\vec\Lambda$ is a diagonal matrix with dataset dependent entries.
For each dataset we optimized the kernel parameters running Carl Rasmussen's minimize function (\url{http://www.gaussianprocess.org/gpml/code/matlab/doc}) for 100 steps.
The initial parameters can be found in Table \ref{tbl:initial_parameters}.
%The performance our approximation is dependent on the hyper-parameters.
The rationale behind 100 steps of optimization is to show an average, examplary picture, summarizing the picture encountered over the whole course of optimization.

\begin{table}
\center
\begin{tabular}{l|r}
\textbf{dataset} & \textbf{properties}\\
\hline
ABALONE
\end{tabular}
\caption{The table of datasets that we used for our experiments.}
\label{tbl:datasets}
\end{table}
\input{tex/evaluation_cg}

\input{tex/discussion}

==> tex/evaluation_cg.tex <==

\subsection{Zero Folds}
DTC gets as much inducing inputs as is feasible in the same number of steps.
\renewcommand{\fsize}{0.3}
\subsubsection{RBF}
\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
%}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~
%}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_0_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
%}
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
%\fbox{
\input{tikz/cg_hybrid_comparison___title_legend__seed_12345.tikz}
%}
\end{subfigure}
%}
}
\caption{Progression of the relative error as a function of the number of iterations of DTC and \kmcg{} for different data-sets using the RBF kernel. 
We used designated training- and test-set where available.
}
\label{fig:cg_hybrid_error_rbf}
\end{figure}

\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_0_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison___title_legend2__seed_12345.tikz}
\end{subfigure}
}
\caption{Progression of the relative error of variance and evidence as a function of the number of iterations of CG and \kmcg{} for different data-sets using the RBF kernel. 
We used designated training- and test-set where available.
}
\label{fig:cg_hybrid_error_rbf_llh}
\end{figure}
\subsubsection{SE}
\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
%}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~
%}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_0_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
%}
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
%\fbox{
\input{tikz/cg_hybrid_comparison___title_legend__seed_12345.tikz}
%}
\end{subfigure}
%}
}
\caption{Progression of the relative error as a function of the number of iterations of DTC and \kmcg{} for different data-sets using the SE kernel. 
We used designated training- and test-set where available.
}
\label{fig:cg_hybrid_error_se}
\end{figure}

\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_0_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison___title_legend2__seed_12345.tikz}
\end{subfigure}
}
\caption{Progression of the relative error of variance and evidence as a function of the number of iterations of CG and \kmcg{} for different data-sets using the SE kernel. 
We used designated training- and test-set where available.
}
\label{fig:cg_hybrid_error_se_llh}
\end{figure}

\subsubsection{Matern}
\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
%}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~
%}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_0_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
%}
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
%\fbox{
\input{tikz/cg_hybrid_comparison___title_legend__seed_12345.tikz}
%}
\end{subfigure}
%}
}
\caption{Progression of the relative error as a function of the number of iterations of DTC and \kmcg{} for different data-sets using the Matern kernel. 
We used designated training- and test-set where available.
}
\label{fig:cg_hybrid_error_matern}
\end{figure}

\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_0_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison___title_legend2__seed_12345.tikz}
\end{subfigure}
}
\caption{Progression of the relative error of variance and evidence as a function of the number of iterations of CG and \kmcg{} for different data-sets using the Matern kernel. 
We used designated training- and test-set where available.
}
\label{fig:cg_hybrid_error_matern_llh}
\end{figure}
 
\subsection{Two Folds}
\subsubsection{RBF}
\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
%}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~
%}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_2_folds_visible_1_covRBF__title_relative_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
%}
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
%\fbox{
\input{tikz/cg_hybrid_comparison___title_legend__seed_12345.tikz}
%}
\end{subfigure}
%}
}
\caption{Progression of the relative error as a function of the number of iterations of DTC and \kmcg{} for different data-sets using the RBF kernel. The data-sets have been mixed.
}
\label{fig:cg_hybrid_error_rbf_mixed}
\end{figure}

\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_2_folds_visible_1_covRBF__title_var_and_nlZ_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison___title_legend2__seed_12345.tikz}
\end{subfigure}
}
\caption{Progression of the relative error of variance and evidence as a function of the number of iterations of CG and \kmcg{} for different data-sets using the RBF kernel. The data-sets have been mixed.
}
\label{fig:cg_hybrid_error_rbf_llh_mixed}
\end{figure}
\subsubsection{SE}
\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
%}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~
%}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_2_folds_visible_1_covSEard__title_relative_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
%}
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
%\fbox{
\input{tikz/cg_hybrid_comparison___title_legend__seed_12345.tikz}
%}
\end{subfigure}
%}
}
\caption{Progression of the relative error as a function of the number of iterations of DTC and \kmcg{} for different data-sets using the SE kernel. The data-sets have been mixed.
}
\label{fig:cg_hybrid_error_se_mixed}
\end{figure}

\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_2_folds_visible_1_covSEard__title_var_and_nlZ_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison___title_legend2__seed_12345.tikz}
\end{subfigure}
}
\caption{Progression of the relative error of variance and evidence as a function of the number of iterations of CG and \kmcg{} for different data-sets using the SE kernel. The data-sets have been mixed.
}
\label{fig:cg_hybrid_error_se_llh_mixed}
\end{figure}

\subsubsection{Matern}
\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
%}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~
%}
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_2_folds_visible_1_covMaternard_5__title_relative_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
%}
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
%\fbox{
\begin{subfigure}[b]{\fsize\textwidth}
\centering
%\fbox{
\input{tikz/cg_hybrid_comparison___title_legend__seed_12345.tikz}
%}
\end{subfigure}
%}
}
\caption{Progression of the relative error as a function of the number of iterations of DTC and \kmcg{} for different data-sets using the Matern kernel. The data-sets have been mixed.
}
\label{fig:cg_hybrid_error_matern_mixed}
\end{figure}

\begin{figure}[H]
\centering
\tempdisable{
\setlength{\figheight}{0.1\textheight}
\setlength{\figwidth}{1.61\figheight}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ABALONE_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ABALONE}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PRECIPITATION_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PRECIPITATION}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_PUMADYN_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{PUMADYN}
\end{subfigure} ~

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MPG_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{MPG}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_MIX_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{TOY DATA}
\end{subfigure} ~
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_POLETELECOMM_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{POLETELECOMM}
\end{subfigure} ~ 

\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_ELEVATORS_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{ELEVATORS}
\end{subfigure} ~ 
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison_AILERONS_folds_2_folds_visible_1_covMaternard_5__title_var_and_nlZ_error__seed_12345.tikz}
\caption{AILERONS}
\end{subfigure} ~ 
\setlength{\figheight}{0.05\textheight}
\setlength{\figwidth}{0.05\textwidth}
\begin{subfigure}[b]{\fsize\textwidth}\centering
\input{tikz/cg_hybrid_comparison___title_legend2__seed_12345.tikz}
\end{subfigure}
}
\caption{Progression of the relative error of variance and evidence as a function of the number of iterations of CG and \kmcg{} for different data-sets using the Matern kernel. The data-sets have been mixed.
}
\label{fig:cg_hybrid_error_matern_llh_mixed}
\end{figure}

\subsection{Grid data}
\subsubsection{RBF}
\subsubsection{SE}
\subsubsection{Matern}
\subsection{Real-time experiments}
We use the same set-up to approach our second question, how much speed-up we obtain. 
Figure \ref{fig:cg_hybrid_times_matern} and \ref{fig:cg_hybrid_times_se} show the accumulated time of each conjugate gradient iteration and set it into relation with the time required for the exact solution.
One can see that the number of steps that our algorithm takes quickly exceeds the time necessary for exact inference before a satisfactory error level could be reached.
Though in theory our algorithm should be faster, in practice Cholesky decomposition is a highly optimized routine which for medium size data-sets it is hard to compete with.
The problem is that we have to evaluate matrix-vector multiplications in a for loop instead of executing one matrix-matrix multiplication\footnote{We implemented our algorithm in Matlab as well as C++ using Eigen. Both implementations are about equally fast.}.
We also ran experiments to see if our approach can be used to speed up \pname{DTC/VFE} and encountered the same problem.


 \setlength{\figheight}{0.04\textheight}
 \setlength{\figwidth}{1.61\figheight}
 \renewcommand{\fsize}{0.3}

\begin{figure}
\center
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_ABALONE_covMaternard_5__title_residual__seed_12345.tikz}
 \centering
 \caption{ABALONE}
 \end{subfigure} ~
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_PRECIPITATION_covMaternard_5__title_residual__seed_12345.tikz}
  \caption{PRECIPITATION}
  \end{subfigure} ~
   \begin{subfigure}[b]{\fsize\textwidth}
   \input{tikz/cg_hybrid_comparison_PUMADYN_covMaternard_5__title_residual__seed_12345.tikz}
   \caption{PUMADYN}
   \end{subfigure} ~
   
    \begin{subfigure}[b]{\fsize\textwidth}
    \input{tikz/cg_hybrid_comparison_MPG_covMaternard_5__title_residual__seed_12345.tikz}
    \caption{MPG}
    \end{subfigure} ~
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_MIX_covMaternard_5__title_residual__seed_12345.tikz}
 \caption{TOY DATA}
 \end{subfigure} ~
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_POLETELECOMM_covMaternard_5__title_residual__seed_12345.tikz}
 \caption{POLETELECOMM}
 \end{subfigure} ~ 
 
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_ELEVATORS_covMaternard_5__title_residual__seed_12345.tikz}
  \caption{ELEVATORS}
  \end{subfigure} ~ 
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_AILERONS_covMaternard_5__title_residual__seed_12345.tikz}
 \caption{AILERONS}
 \end{subfigure} ~ 
\caption{This figure shows the evolution of the residual $||(\vec K+\noise \vec I)\hat{\vec x}-\vec b||_2$ for conjugate gradients and our version over different datasets using the Mat\'ern kernel (Eq.~\ref{eq:matern}).}
\label{fig:cg_hybrid_residual_matern}
\end{figure}

\begin{figure}
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_ABALONE_covSEard__title_residual__seed_12345.tikz}
 \caption{ABALONE}
 \end{subfigure} ~
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_PRECIPITATION_covSEard__title_residual__seed_12345.tikz}
  \caption{PRECIPITATION}
  \end{subfigure} ~
  
   \begin{subfigure}[b]{\fsize\textwidth}
   \input{tikz/cg_hybrid_comparison_PUMADYN_covSEard__title_residual__seed_12345.tikz}
   \caption{PUMADYN}
   \end{subfigure} ~
    \begin{subfigure}[b]{\fsize\textwidth}
    \input{tikz/cg_hybrid_comparison_MPG_covSEard__title_residual__seed_12345.tikz}
    \caption{MPG}
    \end{subfigure} ~
    
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_MIX_covSEard__title_residual__seed_12345.tikz}
 \caption{TOY DATA}
 \end{subfigure} ~
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_POLETELECOMM_covSEard__title_residual__seed_12345.tikz}
 \caption{POLETELECOMM}
 \end{subfigure} ~ 
 
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_ELEVATORS_covSEard__title_residual__seed_12345.tikz}
  \caption{ELEVATORS}
  \end{subfigure} ~ 
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_AILERONS_covSEard__title_residual__seed_12345.tikz}
 \caption{AILERONS}
 \end{subfigure} ~ 
\caption{This figure shows the evolution of the residual $||(\vec K+\noise \vec I)\hat{\vec x}-\vec b||_2$ for conjugate gradients and our version over different datasets using the Mat\'ern kernel (Eq.~\ref{eq:sq_exp}).}
\label{fig:cg_hybrid_residual_se}
\end{figure}

\tempdisable{
\begin{figure}
 \setlength{\figwidth}{0.4\textwidth}
 \setlength{\figheight}{0.25\textwidth}
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_ABALONE_covMaternard_5__title_real_time__seed_12345.tikz}
 \caption{ABALONE}
 \end{subfigure} ~
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_PRECIPITATION_covMaternard_5__title_real_time__seed_12345.tikz}
  \caption{PRECIPITATION}
  \end{subfigure} ~
  
   \begin{subfigure}[b]{\fsize\textwidth}
   \input{tikz/cg_hybrid_comparison_PUMADYN_covMaternard_5__title_real_time__seed_12345.tikz}
   \caption{PUMADYN}
   \end{subfigure} ~
    \begin{subfigure}[b]{\fsize\textwidth}
    \input{tikz/cg_hybrid_comparison_MPG_covMaternard_5__title_real_time__seed_12345.tikz}
    \caption{MPG}
    \end{subfigure} ~
    
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_MIX_covMaternard_5__title_real_time__seed_12345.tikz}
 \caption{TOY DATA}
 \end{subfigure} ~
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_POLETELECOMM_covMaternard_5__title_real_time__seed_12345.tikz}
 \caption{POLETELECOMM}
 \end{subfigure} ~ 
 
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_ELEVATORS_covMaternard_5__title_real_time__seed_12345.tikz}
  \caption{ELEVATORS}
  \end{subfigure} ~ 
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_AILERONS_covMaternard_5__title_real_time__seed_12345.tikz}
 \caption{AILERONS}
 \end{subfigure} ~ 
\caption{This figure shows the accumulated time for each conjugate gradient step on the problem $\vec K\hat{\vec x}\approx \vec b$ for different datasets using the Mat\'ern kernel (Eq.~\ref{eq:matern}).
The straight line is the time of computing the Cholesky decomposition of the full kernel matrix.
}
\label{fig:cg_hybrid_times_matern}
\end{figure}
}

\renewcommand{\fsize}{0.3}
\begin{figure}
 \setlength{\figwidth}{0.4\textwidth}
 \setlength{\figheight}{0.25\textwidth}
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_ABALONE_covSEard__title_real_time__seed_12345.tikz}
 \caption{ABALONE}
 \end{subfigure} ~
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_PRECIPITATION_covSEard__title_real_time__seed_12345.tikz}
  \caption{PRECIPITATION}
  \end{subfigure} ~
  
   \begin{subfigure}[b]{\fsize\textwidth}
   \input{tikz/cg_hybrid_comparison_PUMADYN_covSEard__title_real_time__seed_12345.tikz}
   \caption{PUMADYN}
   \end{subfigure} ~
    \begin{subfigure}[b]{\fsize\textwidth}
    \input{tikz/cg_hybrid_comparison_MPG_covSEard__title_real_time__seed_12345.tikz}
    \caption{MPG}
    \end{subfigure} ~
    
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_MIX_covSEard__title_real_time__seed_12345.tikz}
 \caption{TOY DATA}
 \end{subfigure} ~
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_POLETELECOMM_covSEard__title_real_time__seed_12345.tikz}
 \caption{POLETELECOMM}
 \end{subfigure} ~ 
 
  \begin{subfigure}[b]{\fsize\textwidth}
  \input{tikz/cg_hybrid_comparison_ELEVATORS_covSEard__title_real_time__seed_12345.tikz}
  \caption{ELEVATORS}
  \end{subfigure} ~ 
 \begin{subfigure}[b]{\fsize\textwidth}
 \input{tikz/cg_hybrid_comparison_AILERONS_covSEard__title_real_time__seed_12345.tikz}
 \caption{AILERONS}
 \end{subfigure} ~ 
\caption{This figure shows the accumulated time for each conjugate gradient step on the problem $\vec K\hat{\vec x}\approx \vec b$ for different datasets using the squared-exponential kernel (Eq.~\ref{eq:sq_exp}).
The straight line is the time of computing the Cholesky decomposition of the full kernel matrix.
}

\label{fig:cg_hybrid_times_se}
\end{figure}



%\begin{remark}
%Readers familiar with the theoretical guarantuees of conjugate gradients may be confused that the norm of the residual $||\vec A \hat{\vec x}- \vec y||_2$ does not decrease monotonically.
%However, the guarantees for conjugate gradients refer to $||\vec x - \hat{\vec x}||_{\vec A}$ which is (up to a constant) equivalent to $f(\vec x)\ce\vec x\Trans \vec A \vec x- 2\vec x\Trans \vec b$.
%Conjugate gradients constructs an $\vec x$ that is the minimizer of $f$ in the span of $\vec S$.
%Note that our version of conjugate gradients produces a different $\vec S$, as it solves a different problem (see previous remark).
%%We also looked at the minimizer of $f$ (for $\vec A\ce \vec K + \sigma \vec I$) that is in the span of our $\vec S$.
%%The overall picture remains the same.
%\end{remark}

%Speeding up DTC is not so easy for the same reason. 
%And if it provides a speed-up than Subset of Data is usually better. 
%The Eigenvalue distribution of the kernel matrix is either trivial or hard.
%We could not think of a scenario where it would be favourable for conjugate gradients and at the same time not good for subset of data.
%For some datasets our approach was actually faster but in that case a smaller number of inducing inputs was sufficient to achieve similar performance.
%Therefore we do not reports the results of these experiments here.
